A Grammatical Approach to Data-centric Case Management in a Distributed Collaborative Environment

This paper presents a purely declarative approach to artifact-centric case management systems, and a decentralization scheme for this model. Each case is presented as a tree-like structure; nodes bear information that combines data and computations. Each node belongs to a given stakeholder, and semantic rules govern the evolution of the tree structure, as well as how data values derive from information stemming from the context of the node. Stakeholders communicate through asynchronous message passing without shared memory, enabling convenient distribution.

==> extensions.tex <==

In general, it is not be possible to model a concrete model of case management by a finite set of productions. 
Already in the editorial process of an academic journal we had to resort to production schemas 
of the form  $P=p(\mathbf{x})\langle \mathbf{y}\rangle$ 
where $\mathbf{x}$ is a list of inherited parameters and $\mathbf{y}$ is a list of synthesized parameters. 
The values of synthesized parameters are produced by the pattern matching used for verifying that the (parametric) production 
applies in some open node $X$ of the configuration. At this stage the stakeholder concerned by this node gets the information 
that $p(\mathbf{x})\langle \mathbf{b}\rangle$ is enabled at $X$ where $\mathbf{b}$ is the list of values attached to the 
variables in $\mathbf{y}$ by the pattern matching (some information extracted from the current configuration). 
Then the user may choose to apply a specific instance of this production, by filling in the inherited attributes. 
Namely, a specific set of values $\mathbf{a}$ is assigned to the vector of variables $\mathbf{x}$.
We end up with the actual production $p(\mathbf{a})\langle \mathbf{b}\rangle$, an instance of the parametric production $P$, 
being applied in node $X$. The resulting information $p(\mathbf{a})\langle \mathbf{b}\rangle$ is recorded in the execution log at the given node. 

In order to combine the production and the consumption of attribute values we shall also consider terms with the following mixed notation 
$$t=c(t_1,\ldots,t_n)\langle x_{1},\ldots x_{m}\rangle$$ where constructor $c$ represents some concrete information that can be used to enact 
rules by pattern matching. The terms $t_1,\ldots,t_{n}$ give intentional descriptions of subsequent data.  
The variables $x_{1},\ldots x_{m}$ represent requests for external data needed for the further refinements of $t_1,\ldots,t_{n}$. 
Informally the \textit{data form} $c(t_1,\ldots,t_n)\langle x_{1},\ldots x_{m}\rangle$ represents the data value $c(t_1,\ldots,t_n)$ together 
with the information that the values of $x_1,\ldots,x_m$ are needed at some stage for deriving the values of the terms $t_i$. 

We end up with a uniform notation for services, attribute values, and productions names with respectively sorts, data constructors, and  production names 
ranging in doubly-ranked alphabets.

\begin{definition}\label{def:drAlpha}
A {\bf doubly-ranked alphabet} is a set of constructors $c\in C$ whose arities are given by a pair $(n,m)$ of nonnegative 
integers where $n$ is the number of {\bf arguments} of $c$ and $m$ the number of its {\bf co-arguments}. The set of terms 
over a doubly-ranked alphabet and a set $X$ of variables is given inductively by the following BNF-grammar:
\[
 t ::= x \;\; | \;\; c(t_1,\ldots,t_n)\langle t_{n+1},\ldots t_{n+m}\rangle
\]
where $x\in X$ is a variable and $c$ a constructor of rank $(n,m)$. 
If the set of constructors $C$ is used to build data we define the following two subsets of terms, 
called respectively the {\bf patterns} and the {\bf data}, given by
\[
 \begin{array}{l@{\;\; ::=\;\;}l}
  p & x \;\; | \;\; c(p_1,\ldots,p_n)\langle d_{1},\ldots d_{m}\rangle\\
  d & x \;\; | \;\; c(d_1,\ldots,d_n)\langle x_{1},\ldots x_{m}\rangle
 \end{array}
\]
\DefBox{def:drAlpha}
\end{definition}

\begin{definition}[Extended GAG]\label{def:AW}\mbox{}\\
The productions of an {\bf extended attribute grammar} are of the form:
\[
 P:F_0\;\leftarrow\; F_1 \cdots F_n
\]
Each $F_i$ is a form $s(t_1,\ldots,t_n)\langle u_1,\ldots, u_m\rangle$ where the $t_i$  and the  
$u_j$ are terms over the doubly-ranked alphabet $C$. They respectively provide the values of the inherited attributes 
and of the synthesized attributes (of sort $s$) attached to the form.
$P=p(\mathbf{x})\langle \mathbf{y}\rangle$ is a parametric production consisting of a production name and $\mathbf{x}$ and  
$\mathbf{y}$ are lists of variables with lengths corresponding to the arity of $p$. 
The following transformation when applied to a given production  annotates each of its 
occurrences of variable by a symbol $?$, or $!$. In the former case the occurrence of variable is said to 
be in an {\bf input position} and in the latter case it is said to be in an {\bf output position}. 
\[
 \begin{array}{r@{\;=\;}l}
  !(P:F_0\leftarrow F_1 \cdots F_k) & ?(P):?(F_0) \leftarrow !(F_1) \cdots !(F_k)\\
  ?(p(x_1,\ldots,x_n)\langle y_1,\ldots y_m\rangle & p(?(x_1),\ldots ?(x_n))\langle !(y_1),\ldots !(y_m)\rangle\\
  ?(s(t_1,\ldots t_n)\langle u_1,\ldots u_m\rangle & s(?(t_1),\ldots ?(t_n))\langle !(u_1),\ldots !(u_m)\rangle\\
  !(s(t_1,\ldots t_n)\langle u_1,\ldots u_m\rangle & s(!(t_1),\ldots !(t_n))\langle ?(u_1),\ldots ?(u_m)\rangle\\
  ?(c(t_1,\ldots t_n)\langle u_1,\ldots u_m\rangle & c(?(t_1),\ldots ?(t_n))\langle !(u_1),\ldots !(u_m)\rangle\\
  !(c(t_1,\ldots t_n)\langle u_1,\ldots u_m\rangle & c(!(t_1),\ldots !(t_n))\langle ?(u_1),\ldots ?(u_m)\rangle\\
  ?(x) & x^{?} \\!(x) & x^{!}
 \end{array}
\]
A production is subjected to the following conditions:
\begin{enumerate}
 \item Every variable in a synthesized position of a production name occurs also in an input position of its left-hand side. 
 \item The value of an inherited attribute of the left-hand side is a pattern.
 \item The value of a synthesized attribute in the right-hand side is a variable.
 \item The other values of attributes are data.
 \item Every variable of the production occurs exactly once in an input position.
\end{enumerate}
The \textbf{interface} of the extended attribute grammar is given by a subset of forms 
$F=s(t_1,\ldots,t_n)\langle x_1,\ldots,x_n\rangle$, called its \textbf{services}, 
where the synthesized positions are (distinct) variables $ x_1,\ldots,x_n$.   
\DefBox{def:AW}
\end{definition}

\input{bidirect}

\comment{Traduction de EGAG en GAG. le GAG obtenu est bien form\'e, c'est-\`a-dire sans variables avec des occurrences multiples en entr\'ee si 
l'EGAG v\'erifie restricted single used requirement.}

\comment{Le comportement d'un EGAG est donn\'e par celui du GAG qui lui est associ\'e. N\'eanmoins on peut donner une d\'efinition directe \'equivalente.}

\comment{Adapter (et corriger) la d\'efinition suivante pour qu'elle s'applique aux EGAG.}

\begin{definition}[Applying a Production]\label{def:firingRuleEGAG}
A production $P$ can apply to an open node $X_0$ of a configuration $\Gamma$, 
which we denote as $\netfir{\Gamma}{P/X_0}{}$, 
if the sort $s$ of the left-hand side of $P$ coincides with the sort of $X_0$ and the  
left-hand side of $P$, which is of the form $s(p_1,\ldots,p_n)\langle d'_1,\ldots d'_m\rangle$, matches with 
the form $s(d_1,\ldots,d_n)\langle y_1,\ldots,y_m\rangle$ associated with $X_0$ in $\Gamma$. 
This is the case when each pattern $p_i$ matches with the corresponding data $d_i$ according to the   
(bi-directional) pattern matching given by:
\[
 \begin{array}{l}
  \mathbf{match}(c(p_1,\ldots,p_n)\langle d_1,\ldots,d_m\rangle,c(d_1,\ldots,d_n)\langle x_1,\ldots,x_m\rangle \\
  \qquad\qquad=
  \setof{x_i=d_i}{1\leq i\leq n}+\sum_{i=1}^{n} \mathbf{match}(p_i,d_i)\\
   \mathbf{match}(x,d) = \set{x=d}
 \end{array}
\]
where we  assume $\mathit{var}(P)\cap\mathit{var}(\Gamma)=\emptyset$ (up to a renaming of the variables in $P$) 
and where the sum $\sigma =\sum_i \sigma_i$ of substitutions $\sigma_i$ is defined when each of the substitutions $\sigma_i$ is defined 
and they are associated with disjoint sets of variables, in that case the resulting substitution is their union: $\sigma=\bigcup_i \sigma_i$.

When $P$ applies in $X_0$, i.e. the left-hand side $s(p_1,\ldots,p_n)\langle d'_1,\ldots d'_m\rangle$ 
of $P$ matches with the form $s(d_1,\ldots,d_n)\langle y_1,\ldots,y_m\rangle$ associated with $X_0$, we let 
$\sigma_{\mathit{in}}$ and $\sigma_{\mathit{out}}$ denote the substitutions given by 
$\sigma_{\mathit{in}}=\sum_{i=1}^{n} \mathbf{match}(p_i,d_i)$ and 
$\sigma_{\mathit{out}}=\setof{y_j=d'_j\sigma_{\mathit{in}}}{1\leq j\leq m}$. 

Applying production $P=F\leftarrow F_1\ldots F_k$ in $X_0$ transforms configuration $\Gamma$ 
into  $\Gamma'$, denoted as  $\netfir{\Gamma}{P/X_0}{\Gamma'}$, where\vspace{-1mm}:
\[
  \begin{array}{rcl}
   \Gamma' & = & \set{X_0=P(X_1,\ldots,X_k)}\qquad \mbox{where}\quad X_1,\ldots,X_k\quad\mbox{are new nodes added to $\Gamma'$}\\
           & \cup & \set{X_1=F_1\sigma_{\mathit{in}}, \ldots, X_k=F_k\sigma_{\mathit{in}}} \\
           & \cup & \setof{X=F\sigma}{(X=F)\in\Gamma\;\wedge\; X\neq X_0}
  \end{array}\vspace{-1mm}
\]
with $\sigma =\sigma_{\mathit{in}}\cup\sigma_{\mathit{out}}$. 
\DefBox{def:firingRuleEGAG}
\end{definition}

\input{bidirect2}
